Do I Get the Privacy I Need? Benchmarking Utility in Differential Privacy Libraries

An increasing number of open-source libraries promise to bring differential privacy to practice, even for non-experts. This paper studies five libraries that offer differentially private analytics: Google DP, SmartNoise, diffprivlib, diffpriv, and Chorus. We compare these libraries qualitatively (capabilities, features, and maturity) and quantitatively (utility and scalability) across four analytics queries (count, sum, mean, and variance) executed on synthetic and real-world datasets. We conclude that these libraries provide similar utility (except in some notable scenarios). However, there are significant differences in the features provided, and we find that no single library excels in all areas. Based on our results, we provide guidance for practitioners to help in choosing a suitable library, guidance for library designers to enhance their software, and guidance for researchers on open challenges in differential privacy tools for non-experts.

==> Experiment_results.tex <==
\begin{table*}
\centering
\footnotesize
\begin{tabular}{ |M{2cm}||M{2.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}| } 

\hline
\textbf{Features}  & \textbf{diffprivlib} & \textbf{SmartNoise} & \textbf{PyDP \break (Google-DP)} & \textbf{diffpriv} & \textbf{Chorus}\\
\hline\hline

\multicolumn{6}{|l|}{\textit{Accuracy results "Risk neutral"/"Risk averse"}}\\
\cline{1-6}
Count & $1^{st}$/  &  $2^{nd}$/ & $3^{rd}$/  &  $4^{th}$/ &  $5^{th}$/ \\
\hline
Sum &  / & /  & / & /  & / \\
\hline
Mean &  / &  / & / & /  & / \\
\hline
Var & /  & /  & / & /  & / \\
\hline

\multicolumn{6}{|l|}{\textit{Throughput results}}\\
\cline{1-6}
Count & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
Sum & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$  \\
\hline
Mean & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
Var & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline

\multicolumn{6}{|l|}{\textit{Memory consumption results}}\\
\cline{1-6}
Count & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
Sum & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$  \\
\hline
Mean & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
Var & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline


\end{tabular}

\caption{Experiments results in terms of accuracy, throughput, and memory consumption. \break *With sensitivity sampler.} 
\label{tab:Experiments_Table}

\end{table*}

\begin{comment}
\multicolumn{6}{|l|}{\textit{Operational ranking:}}\\
\cline{1-6}
Throughput & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
Memory consumption  & $1^{st}$  &  $2^{nd}$ & $3^{rd}$  &  $4^{th}(5^{th*})$ &  $5^{th}$ \\
\hline
\end{comment}

==> results_table.tex <==



% % %\begin{landscape}

% % \footnotesize
% % \begin{tabularx}{\linewidth}{%

% % \end{tabularx}

% % %\end{landscape}


% \begin{table*}

% \begin{centering}
% %\begin{adjustbox}{width=1\textwidth}
% \footnotesize

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{3}{|c|}{\textbf{Query}} & \multicolumn{5}{c|}{\textbf{Count}} & \multicolumn{5}{c|}{\textbf{Sum}} & \multicolumn{5}{c|}{\textbf{Mean}} & \multicolumn{5}{c|}{\textbf{Variance}} \\ \hline
% \multicolumn{3}{|c|}{\textbf{}{Library}} & \multicolumn{1}{c|}{diffprivlib} & \multicolumn{1}{c|}{smartnoise} & 
% \multicolumn{1}{c|}{pydp} & 
% \multicolumn{1}{c|}{diffpriv} & 
% \multicolumn{1}{c|}{chorus} &
% \multicolumn{1}{c|}{diffprivlib} & \multicolumn{1}{c|}{smartnoise} & 
% \multicolumn{1}{c|}{pydp} & 
% \multicolumn{1}{c|}{diffpriv} & 
% \multicolumn{1}{c|}{chorus} &
% \multicolumn{1}{c|}{diffprivlib} & \multicolumn{1}{c|}{smartnoise} & 
% \multicolumn{1}{c|}{pydp} & 
% \multicolumn{1}{c|}{diffpriv} &
% \multicolumn{1}{c|}{chorus} &
% \multicolumn{1}{c|}{diffprivlib} & \multicolumn{1}{c|}{smartnoise} & 
% \multicolumn{1}{c|}{pydp} & 
% \multicolumn{1}{c|}{diffpriv} &
% \multicolumn{1}{c|}{chorus} \\ \hline
%  \multirow{6}{*}{{\rotatebox[origin=c]{90}{\textbf{Risk-Neutral}}} {\rotatebox[origin=c]{90}{$\reallywidehat{RE}$}}} & \multirow{2}{*}{$\varepsilon$ \textless 1} & mean & 4.207e-05 & \textbf{3.192e-07} & 2.931e-06 & 5.370e-07 & -  & 9.911e-06 & 9.462e-07 & 3.300e-06 & \textbf{1.285e-08} & -& 4.217e-06 & 1.269e-06 & 1.804e-06 & \textbf{1.299e-08} & -& 0.0002 & 0.0001 & 0.0001 & \textbf{1.595e-10} & - \\ %\cline{3-19} 
%  &  & std &  7.534e-05 & 7.847e-06 &  1.465e-05 & \textbf{5.464e-06} & - & 5.884e-05 & 2.561e-05 & 5.329e-05 & \textbf{6.528e-08} & -& 6.088e-05 & 5.371e-05 & 4.781e-05 & \textbf{8.412e-08} & -& 0.0017 & 0.0008 & 0.0017 & \textbf{1.374e-09} & - \\ %\cline{2-19} 
 
%  & \multirow{2}{*}{1\textless $\varepsilon$ \textless 10} & mean & 6.420e-07 & \textbf{2.800e-08} & 3.800e-08 & 5.301e-08 &-& 1.171e-07 & 6.014e-07 & 1.835e-07 & \textbf{8.964e-10} & -& 1.351e-07 & 2.576e-07 & 2.617e-07 & \textbf{3.716e-10} & -& 1.357e-06 & 9.799e-06 & 3.105e-05 & \textbf{3.813e-12} & - \\ %\cline{3-19} 
%  &  & std & 1.244e-06 & 1.585e-07 & \textbf{1.578e-07} & 2.316e-07 & - & 1.674e-06 & 1.062e-06 & 8.674e-07 & \textbf{2.264e-09} & -& 1.092e-06 & 8.109e-07 & 6.452e-07 & \textbf{9.595e-10} & -& 1.478e-05 & 1.204e-05 & 5.463e-05 & \textbf{1.616e-11} & -\\ %\cline{2-19} 
 
%  & \multirow{2}{*}{10\textless $\varepsilon$ \textless 100} & mean & \textbf{0.0} & 0.0 & 0.0 & 3.948e-09 &-& 5.084e-08 & 4.755e-08 & 3.392e-08 & \textbf{5.757e-11} & -& 8.842e-08 & 2.984e-08 & 3.192e-08 & \textbf{6.581e-11} & -& 4.978e-07 & 1.013e-05 & 1.380e-06 & \textbf{1.125e-13} & -\\ %\cline{3-19} 
%  &  & std & \textbf{0.0} & 0.0 & 0.0 & 1.747e-08 &-& 7.776e-08 & 5.502e-08 & 2.372e-08 & \textbf{1.742e-10} & -& 1.477e-07 & 1.205e-07 & 1.023e-07 & \textbf{1.192e-10} & -& 1.009e-06 & 1.239e-06 & 3.235e-06 & \textbf{2.519e-12} & -\\ \hline
 
 
 
%  \multirow{6}{*}{{\rotatebox[origin=c]{90}{\textbf{Risk-Averse}}} {\rotatebox[origin=c]{90}{$S$}}}& \multirow{2}{*}{$\varepsilon$ \textless 1} & mean & \textbf{7.217e-05} & 0.00012 & 0.00012 & 0.00011 &-& 0.275 & 0.282 & 0.265 & \textbf{0.0005} & - & 2.723e-06 & 2.778e-06 & 3.273e-06 & \textbf{5.217e-09} & -& 0.0123 & 0.0066 & 0.0172 & \textbf{1.288e-08} & - \\ %\cline{3-19} 
%  &  & std & \textbf{0.00012} & 0.00021 & 0.00022 & 0.0002 &-& 0.502 & 0.4905 & 0.456 & \textbf{0.0009} & -& 4.873e-06 & 4.854e-06 & 6.078e-06 & \textbf{9.341e-09} & -& 0.0236 & 0.0127 & 0.0305 & \textbf{2.448e-08} & -\\ %\cline{2-19} 
 
%  & \multirow{2}{*}{1\textless $\varepsilon$ \textless 10} & mean &  \textbf{1.799e-06} & 2.721e-06 & 4.116e-06 & 4.130e-06 &-& 0.0095 & 0.010 & \textbf{0.0093} & 1.845 & -& 9.551e-08 & 9.423e-08 & 1.119e-07 & \textbf{1.800e-10} & -& 0.00028 & 0.0002 & 0.0005 & \textbf{4.334e-10} & -\\ %\cline{3-19} 
%  &  & std & \textbf{2.454e-06} & 4.119e-06 & 4.147e-06 & 3.630e-06 &-& 0.0086 & 0.0089 & \textbf{0.0081} & 1.6531 & -& 8.944e-08 & 8.111e-08 & 9.794e-08 & \textbf{1.639e-10} & -& 0.0003 & 0.0002 & 0.0005 & \textbf{3.927e-10} & - \\ %\cline{2-19} 
 
%  & \multirow{2}{*}{10\textless $\varepsilon$ \textless 100} & mean &  \textbf{0.0} & 0.0 & 0.0 & 3.041e-07 &-& 0.00069 & 0.00072 & \textbf{0.00066} & 1.3395 & -& 7.035e-09 & 7.266e-09 & 8.124e-09 & \textbf{1.332e-11} & -& 1.632e-05 & 1.6412e-05 & 4.228e-05 & \textbf{3.222e-11} & -\\ %\cline{3-19} 
%  &  & std & \textbf{0.0} & 0.0 & 0.0 & 1.849e-07 &-& \textbf{0.00038} & 0.00042 & 0.00038 & 8.4326 & -& 4.260e-09 & 4.121e-09 & 4.559e-09 & \textbf{7.247e-12} & -& 9.603e-06 & 9.604e-06 & 2.283e-05 & \textbf{1.901e-11} & - \\ \hline
 
 
  
%  \multirow{4}{*}{{\rotatebox{90}{\textbf{Execution}}} {\rotatebox[origin=l]{90}{time}}}& \multirow{2}{*}{10 - 10k} & mean & 0.0017 & 0.0156 & \textbf{0.00018} & 0.00063 &-& 0.0018 & 0.0169 & \textbf{0.0003} & 0.0009 & -& 0.0017 & 0.0142 & \textbf{0.0003} & 0.0007 & -& 0.004 & 0.0146 & \textbf{0.0004} & 0.0008 & -\\ %\cline{3-19} 
%  &  & std & 0.0014 & 0.0247 & \textbf{0.0001} & 5.5497 &-& 0.0016 & 0.026 & \textbf{0.0001} & 0.0004 & -& 0.0016 & 0.0209 & \textbf{0.0001} & 0.0002 & -& 0.0021 & 0.0218 & \textbf{0.0001} & 0.0004 & -\\ %\cline{2-19} 
 
%  & \multirow{2}{*}{100k - 100 mil} & mean & 1.8785 & 5242.9083 & \textbf{0.0002} & 0.00106 &-&144.232  & 1130.578 & \textbf{0.00038} & 0.1295 & -& 132.313 & 178.161 & \textbf{0.0004} & 0.2727 & -& 30.659 & 8414.199 & \textbf{0.00049} & 0.4729& -\\ %\cline{3-19} 
%  &  & std & 2.5491 & 7412.41 & \textbf{0.0001} & 0.0007 &-& 203.875 & 1596.733 & \textbf{0.0002} & 0.1748 & -& 187.022 & 249.756 & \textbf{0.0002} & 0.3699 & -& 43.22 & 11897.16 & \textbf{0.0003} & 0.6395 & - \\ \hline
 
  
%  \multirow{4}{*}{{\rotatebox{90}{\textbf{Memory}}} {\rotatebox[origin=l]{90}{consumption}}}& \multirow{2}{*}{10 - 10k} & mean & 90458521 & 73895116 & \textbf{57683148} & - &-& 90338099 & 74716774 & \textbf{57307955} & - & -& 90331545 & \textbf{72025702} & 861637290 & - & -& 90423296 & 74344038 & \textbf{57430835} & - & -\\ %\cline{3-19} 
%  &  & std & 16927910 & 5700165 & \textbf{5623464} & - &-& 16811555 & 6193761 & \textbf{5295729} & - & -& 16809457 & \textbf{1986087} & 5404328 & - & -& 16732519 & 5886528 & \textbf{5311916} & - & -\\ %\cline{2-19} 
 
%  & \multirow{2}{*}{100k - 100 mil} & mean & 906844842 & 3249827840 & \textbf{861973162} & - &-& 881292629 & 3250672981 & \textbf{861491200} & - & -& 881248938 & \textbf{196636672} & 861637290 & - & -& 881222997 & 3248772437 & \textbf{861551274} & -& - \\ %\cline{3-19} 
%  &  & std & 1048973990 & 4164865713 & \textbf{1038735693} & - &-& \textbf{1007203265} & 4165383198 & 1039041472 & - & -& 1007147316 & \textbf{194071240} & 1038802203 & - & -& \textbf{1007026669} & 4163052758 & 1038941133 & - & - \\ \hline
 

% \end{tabular}%
% %\end{adjustbox}

% \label{tab:Accuracy_Performance_results}
% \caption{Summary table containing the experiments' accuracy and performance results for the different analytics queries executed on a normally distributed synthetic datasets. For accuracy, the scale of the dataset was of 10000 data points, std of 250 and skew of 5; while for performance, the scale varied in the given intervals of the table with the same std and skewness as for the accuracy results.}

% \end{centering}
% \end{table*}





